Evolving generalist controllers to handle a wide range of morphological variations

Neuro-evolutionary methods have proven effective in addressing a wide range of tasks. However, the study of the robustness and generalizability of evolved artificial neural networks (ANNs) has remained limited. This has immense implications in the fields like robotics where such controllers are used in control tasks. Unexpected morphological or environmental changes during operation can risk failure if the ANN controllers are unable to handle these changes. This paper proposes an algorithm that aims to enhance the robustness and generalizability of the controllers. This is achieved by introducing morphological variations during the evolutionary training process. As a results, it is possible to discover generalist controllers that can handle a wide range of morphological variations sufficiently without the need of the information regarding their morphologies or adaptation of their parameters. We perform an extensive experimental analysis on simulation that demonstrates the trade-off between specialist and generalist controllers. The results show that generalists are able to control a range of morphological variations with a cost of underperforming on a specific morphology relative to a specialist. This research contributes to the field by addressing the limited understanding of robustness and generalizability and proposes a method by which to improve these properties.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/supplementaryInfo.tex <==


\section{Fitness trends during the evolutionary processes}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.55\textwidth]{figures/evolutionaryRuns.pdf}
    \caption{Illustration of fitness values of five independent evolutionary processes (on morphology size of 64) on four problems.}
    \label{fig:evolutionaryRuns}
\end{figure*}

Figure~\ref{fig:evolutionaryRuns} shows the fitness trends during the evolutionary processes on four agent types. In CartPole, evolutionary branching was not observed. A single generalist controller is learned less than 100 generations. In other environments, we can observe occasional fitness increase that indicate the restart of the evolutionary process that is run on the outlier sets. 

\section{Evolutionary branching}
Table~\ref{tab:clusters} shows the average number of evolutionary branching (and standard deviation) observed based on the size of training morphologies in each problem type. CartPole did not show any branching, whereas Walker2D showed the largest number of branching. In Figure~\ref{fig:visual_alg}, illustrate the branching process and how it partitions the space of morphology variations.

\begin{table*}[ht!]
\centering
\caption{Table shows the mean and standard deviation of the number of clusters for each combination of environment and size of the training morphology set.}\label{tab:clusters}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}l@{}}\textbf{Size of training morphologies:}\end{tabular} & \textbf{1} & \textbf{16}  & \textbf{25}  & \textbf{49} & \textbf{64}                                                      \\ \hline
\textbf{CartPole}                                                                                      & \begin{tabular}[c]{@{}c@{}}1 \end{tabular} & \begin{tabular}[c]{@{}c@{}}1   \end{tabular}       & \begin{tabular}[c]{@{}c@{}}1   \end{tabular}        & \begin{tabular}[c]{@{}c@{}}1   \end{tabular}        & \begin{tabular}[c]{@{}c@{}}1   \end{tabular}       \\ \hline
\textbf{Bipedal Walker}                                                                                & \begin{tabular}[c]{@{}c@{}}1   \end{tabular} & \begin{tabular}[c]{@{}c@{}}1.67   $\pm$ 0.96\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.367   $\pm$ 0.56\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.367   $\pm$ 0.61\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.53   $\pm$ 0.78\end{tabular}  \\ \hline
\textbf{Ant}                                                                                          & \begin{tabular}[c]{@{}c@{}}1   \end{tabular} & \begin{tabular}[c]{@{}c@{}}1.67   $\pm$ 0.84\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.7   $\pm$ 0.92\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.9  $\pm$ 1.12\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2.33   $\pm$ 1.24\end{tabular} \\ \hline
\textbf{Walker2D}                                                                                      & \begin{tabular}[c]{@{}c@{}}1   \end{tabular} & \begin{tabular}[c]{@{}c@{}}2.4   $\pm$ 1.04\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.9   $\pm$ 0.99\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.2   $\pm$ 1.06\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.1   $\pm$ 1.24\end{tabular}  \\ \hline
\end{tabular}
\end{table*}


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=.8\linewidth]{figures/visual_alg.pdf}
    \caption{Visualization of an example of the evolutionary branching. The algorithm starts with an empty set $G$ and a morphology set $M_1$ which results in a controller $I_1$ and a set of left-over morphologies $M_2$. $I_1$ is added to $G$ and the evolution restarts with $M_2$. This repeats until enough  controllers $I$ have been found that together cover the morphology space and have been added to $G$. Overall, the process partitions the morphological space into clusters that can be controlled by generalist controllers as much as possible. } 
    \label{fig:visual_alg}
\end{figure*}

